Parabolic problem with fractional time derivative with nonlocal and nonsingular Mittag-Leffler kernel

We prove H\"older regularity results for a class of nonlinear parabolic problem with fractional-time derivative with nonlocal and Mittag-Leffler nonsingular kernel. Existence of weak solutions via approximating solutions is proved. Moreover, the H\"{o}lder continuity of viscosity solutions is obtained. We get the similar results as those obtained by Allen (see {\url{https://arxiv.org/abs/1610.10073}})

==> DAI_commands.tex <==
\renewcommand{\L}{\mathcal{L}}
\newcommand{\R}{  \mathbb{R}}
\newcommand{\C}{  \mathcal{C}}
\newcommand{\Q}{  \mathbb{Q}}
\newcommand{\N}{  \mathbb{N}}
\renewcommand{\P}{ \mathbb{P}}
\newcommand{\V}{  \mathbb{V}}
\newcommand{\E}{  \mathbb{E}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\DC}{ {}^{C}\D_{a}^{\alpha}}
\newcommand{\AB}{ {}^{ABC}\D_{a}^{\alpha}}
\newcommand{\fiab}[2]{\prescript{\text{AB}}{#1} I_{t}^{#2}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\K}{{\mathcal K}}
\newcommand{\M}{{\mathcal M}}
%----------------------------
%Vektorbuchstaben
\newcommand{\vX}{\mathbf{X}}
\newcommand{\vY}{\mathbf{Y}}
\newcommand{\vZ}{\mathbf{Z}}
\newcommand{\vW}{\mathbf{W}}
\newcommand{\vS}{\mathbf{S}}
\newcommand{\va}{\mathbf{a}}
\newcommand{\vb}{\mathbf{b}}
\newcommand{\vc}{\mathbf{c}}
\newcommand{\vsigma}{\mathbf{\sigma}}
\newcommand{\vbeta}{\mathbf{\beta}}
\newcommand{\vmu}{\mathbf{\mu}}
\newcommand{\vtheta}{\mathbf{\theta}}
\newcommand{\vs}{\mathbf{s}}
\newcommand{\vx}{\mathbf{x}}
%-------------------------------------
\newcommand{\cA}{  \mathcal{A}}
\newcommand{\cB}{  \mathcal{B}}
\newcommand{\cC}{  \mathcal{C}}
\newcommand{\cD}{  \mathcal{D}}
\newcommand{\cE}{  \mathcal{E}}
\newcommand{\cF}{  \mathcal{F}}
\newcommand{\cG}{  \mathcal{G}}
\newcommand{\cH}{  \mathcal{H}}
\newcommand{\cI}{  \mathcal{I}}
\newcommand{\cJ}{  \mathcal{J}}
\newcommand{\cK}{  \mathcal{K}}
\newcommand{\cL}{  \mathcal{L}}
\newcommand{\cM}{  \mathcal{M}}
\newcommand{\cN}{  \mathcal{N}}
\newcommand{\cO}{  \mathcal{O}}
\newcommand{\cP}{  \mathcal{P}}
\newcommand{\cQ}{  \mathcal{Q}}
\newcommand{\cR}{  \mathcal{R}}
\newcommand{\cS}{  \mathcal{S}}
\newcommand{\cT}{  \mathcal{T}}
\newcommand{\cU}{  \mathcal{U}}
\newcommand{\cV}{  \mathcal{V}}
\newcommand{\cW}{  \mathcal{W}}
\newcommand{\cX}{  \mathcal{X}}
\newcommand{\cY}{  \mathcal{Y}}
\newcommand{\cZ}{  \mathcal{Z}}
%-----------------------------------
\newcommand{\fA}{  \mathfrak{A}}
\newcommand{\fB}{  \mathfrak{B}}
\newcommand{\fC}{  \mathfrak{C}}
\newcommand{\fD}{  \mathfrak{D}}
\newcommand{\fE}{  \mathfrak{E}}
\newcommand{\fF}{  \mathfrak{F}}
\newcommand{\fG}{  \mathfrak{G}}
\newcommand{\fH}{  \mathfrak{H}}
\newcommand{\fI}{  \mathfrak{I}}
\newcommand{\fJ}{  \mathfrak{J}}
\newcommand{\fK}{  \mathfrak{K}}
\newcommand{\fL}{  \mathfrak{L}}
\newcommand{\fM}{  \mathfrak{M}}
\newcommand{\fN}{  \mathfrak{N}}
\newcommand{\fO}{  \mathfrak{O}}
\newcommand{\fP}{  \mathfrak{P}}
\newcommand{\fQ}{  \mathfrak{Q}}
\newcommand{\fR}{  \mathfrak{R}}
\newcommand{\fS}{  \mathfrak{S}}
\newcommand{\fT}{  \mathfrak{T}}
\newcommand{\fU}{  \mathfrak{U}}
\newcommand{\fV}{  \mathfrak{V}}
\newcommand{\fW}{  \mathfrak{W}}
\newcommand{\fX}{  \mathfrak{X}}
\newcommand{\fY}{  \mathfrak{Y}}
\newcommand{\fZ}{  \mathfrak{Z}}
%-------------------------------

\renewcommand{\epsilon}{\varepsilon}

%-------------------------------

\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\Supp}{supp}
%-----------------------------

\newcommand{\norm}[1]{\left\| #1 \right\|}

\newcommand{\bet}[1]{\left| #1 \right|}

\newcommand{\ska}[1]{\left\langle #1 \right\rangle}

\newcommand{\wkonv}[1]{\overset{#1 \to \infty}{\Longrightarrow}}

\newcommand{\konv}[1]{\overset{#1 \to \infty}{\longrightarrow}}

\newcommand{\vertkonv}{\overset{\cD}{\longrightarrow}}

\newcommand{\Ind}[1]{\ensuremath \mathbbm{1}_{#1}}
\newcommand{\W}{\ensuremath \mathbb{W}}
\newcommand{\floor}[1]{\ensuremath \left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\ensuremath \left\lceil #1 \right\rceil}
\newcommand{\td}{d^\circ}
\renewcommand{\iff}{\Leftrightarrow}
\renewcommand{\d}{\text{d}}
\newcommand{\ortho}{\mathcal{O}}


